RadGraph: Extracting Clinical Entities and Relations from Radiology Reports

Extracting structured clinical information from free-text radiology reports can enable the use of radiology report information for a variety of critical healthcare applications. In our work, we present RadGraph, a dataset of entities and relations in full-text chest X-ray radiology reports based on a novel information extraction schema we designed to structure radiology reports. We release a development dataset, which contains board-certified radiologist annotations for 500 radiology reports from the MIMIC-CXR dataset (14,579 entities and 10,889 relations), and a test dataset, which contains two independent sets of board-certified radiologist annotations for 100 radiology reports split equally across the MIMIC-CXR and CheXpert datasets. Using these datasets, we train and test a deep learning model, RadGraph Benchmark, that achieves a micro F1 of 0.82 and 0.73 on relation extraction on the MIMIC-CXR and CheXpert test sets respectively. Additionally, we release an inference dataset, which contains annotations automatically generated by RadGraph Benchmark across 220,763 MIMIC-CXR reports (around 6 million entities and 4 million relations) and 500 CheXpert reports (13,783 entities and 9,908 relations) with mappings to associated chest radiographs. Our freely available dataset can facilitate a wide range of research in medical natural language processing, as well as computer vision and multi-modal learning when linked to chest radiographs.

==> tables/top_entities.tex <==
% \usepackage{booktabs}
% \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
% \caption{Top 20 entities in train set by type}
% \label{top-entities}

\begin{table}[hbt!]
\caption{Top entities in train set}
\label{top-entities}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrlrlrlr} 
\toprule
\multicolumn{2}{c}{\textit{Anatomy}}        & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textit{Observation:}\\\textit{definitely present}\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textit{Observation:}\\\textit{uncertain}\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textit{Observation:}\\\textit{definitely absent}\end{tabular}}  \\ 
\cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Entity            & \%                      & Entity        & \%                                                                                             & Entity         & \%                                                                                   & Entity         & \%                                                                                            \\ 
\midrule
right*            & 8.3                     & effusion*     & 4.3                                                                                            & atelectasis*   & 9.7                                                                                  & pneumothorax*  & 18.8                                                                                          \\
pleural*          & 8.0                     & normal*       & 3.9                                                                                            & effusion*      & 7.7                                                                                  & effusion*      & 14.0                                                                                          \\
left*             & 7.3                     & unchanged*    & 3.8                                                                                            & pneumonia*     & 7.3                                                                                  & consolidation* & 8.1                                                                                           \\
lung*             & 6.4                     & opacity*      & 3.4                                                                                            & infection      & 4.9                                                                                  & acute          & 7.8                                                                                           \\
pulmonary*        & 5.2                     & tube*         & 3.0                                                                                            & edema*         & 4.6                                                                                  & focal          & 7.3                                                                                           \\
silhouette*       & 2.7                     & atelectasis*  & 3.0                                                                                            & small*         & 4.4                                                                                  & pneumonia*     & 4.6                                                                                           \\
heart*            & 2.4                     & mild*         & 2.8                                                                                            & aspiration     & 3.1                                                                                  & edema*         & 4.5                                                                                           \\
size*             & 2.4                     & small*        & 2.6                                                                                            & mild*          & 2.9                                                                                  & process        & 3.7                                                                                           \\
cardiac           & 2.2                     & moderate      & 2.4                                                                                            & consolidation* & 2.4                                                                                  & abnormality    & 3.3                                                                                           \\
lower             & 2.2                     & stable        & 2.3                                                                                            & infectious     & 1.9                                                                                  & opacity*       & 1.4                                                                                           \\
mediastinal       & \multicolumn{1}{l}{2.2} & clear         & 2.0                                                                                            & pneumothorax*  & 1.5                                                                                  & new            & 1.4                                                                                           \\
contour           & 2.1                     & edema*        & 1.8                                                                                            & hemorrhage     & 1.4                                                                                  & change         & 1.4                                                                                           \\
bilateral         & 2.0                     & tip           & 1.6                                                                                            & underlying     & 1.4                                                                                  & tube*          & 1.4                                                                                           \\
lobe              & 1.8                     & cardiomegaly  & 1.4                                                                                            & superimposed   & 1.2                                                                                  & large          & 1.3                                                                                           \\
volume            & 1.8                     & increased     & 1.2                                                                                            & chronic        & 1.2                                                                                  & congestion     & 1.2                                                                                           \\
vascular          & 1.6                     & low           & 1.1                                                                                            & scarring       & 1.2                                                                                  & fracture       & 0.9                                                                                           \\
cardiomediastinal & 1.6                     & line          & 1.0                                                                                            & process        & 1.0                                                                                  & overt          & 0.8                                                                                           \\
upper             & 1.5                     & congestion    & 1.0                                                                                            & fluid          & 1.0                                                                                  & air            & 0.8                                                                                           \\
hilar             & 1.3                     & new           & 1.0                                                                                            & focal          & 1.0                                                                                  & free           & 0.7                                                                                           \\
chest             & 1.1                     & pneumothorax* & 1.0                                                                                            & early          & 0.9                                                                                  & displaced      & 0.6                                                                                           \\ 
\midrule
\multicolumn{8}{l}{\textit{* Top 20 entities across all types.}}                                                                                                                                                                                                                                                                                                                      \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/top_relations.tex <==
% \usepackage{booktabs}
% \cmidrule(lr){1-3}\cmidrule(lr){4-6}\cmidrule(lr){7-9}
% \caption{Top 20 relations in train set by type}
% \label{top-relations}

\begin{table}[hbt!]
\caption{Top relation pairs in train set}
\label{top-relations}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{llrllrllr} 
\toprule
\multicolumn{3}{c}{\textit{modify}}    & \multicolumn{3}{c}{\textit{located at}}  & \multicolumn{3}{c}{\textit{suggestive of}}  \\ 
\cmidrule(lr){1-3}\cmidrule(lr){4-6}\cmidrule(lr){7-9}
Subject     & Object             & \%  & Subject       & Object            & \%   & Subject       & Object        & \%          \\ 
\midrule
small*      & effusion*          & 1.7 & effusion*     & pleural*          & 12.2 & opacity       & atelectasis   & 11.6        \\
size*       & heart*             & 1.7 & edema*        & pulmonary*        & 4.3  & opacity       & pneumonia     & 7.2         \\
silhouette* & cardiac*           & 1.5 & clear*        & lung*             & 3.0  & opacity       & infection     & 4.6         \\
focal*      & consolidation*     & 1.5 & normal*       & heart*            & 2.2  & consolidation & pneumonia     & 4.6         \\
right*      & pleural*           & 1.3 & congestion*   & vascular*         & 2.1  & opacity       & aspiration    & 2.8         \\
volume*     & lung*              & 1.3 & low           & lung              & 1.5  & opacity       & edema         & 1.9         \\
left*       & pleural*           & 1.2 & normal        & cardiomediastinal & 1.4  & blunting      & effusion      & 1.6         \\
lower*      & lobe*              & 1.2 & opacity       & lung              & 1.3  & marking       & edema         & 1.6         \\
bilateral*  & pleural*           & 1.1 & process       & cardiopulmonary   & 1.3  & low           & crowding      & 1.4         \\
contour*    & mediastinal*       & 1.1 & atelectasis   & bibasilar         & 1.2  & consolidation & atelectasis   & 1.2         \\
left*       & lung*              & 1.0 & normal        & hilar             & 1.1  & opacity       & effusion      & 1.2         \\
moderate*   & effusion*          & 1.0 & normal        & mediastinal       & 1.1  & opacification & effusion      & 0.9         \\
contour*    & hilar*             & 1.0 & fracture      & rib               & 1.0  & opacity       & scarring      & 0.9         \\
right*      & lung*              & 0.9 & consolidation & lung              & 1.0  & opacity       & consolidation & 0.9         \\
silhouette* & cardiomediastinal* & 0.9 & tube          & chest             & 0.9  & opacification & fluid         & 0.9         \\
left        & lobe               & 0.9 & abnormality   & osseous           & 0.9  & opacity       & hemorrhage    & 0.9         \\
acute       & process            & 0.8 & pneumothorax  & apical            & 0.9  & consolidation & aspiration    & 0.7         \\
mild        & edema              & 0.8 & opacity       & lobe              & 0.8  & opacity       & fluid         & 0.7         \\
right       & lobe               & 0.8 & normal        & cardiac           & 0.8  & enlarged      & hypertension  & 0.5         \\
tip         & tube               & 0.7 & edema         & interstitial      & 0.8  & prominence    & hypertension  & 0.5         \\ 
\midrule
\multicolumn{9}{l}{\textit{* Top 20 relations across all types.}}                                                               \\
\bottomrule
\end{tabular}
}
\end{table}
